Problems of dataset creation for light source estimation

The paper describes our experience collecting a new dataset for the light source estimation problem in a single image. The analysis of existing color targets is presented along with various technical and scientific aspects essential for data collection. The paper also contains an announcement of an upcoming 2-nd International Illumination Estimation Challenge (IEC 2020).

==> chapters/collecting_with_cube.tex <==
\section{Notes on the dataset collection in uncontrolled conditions}

\ruengtext{
Для сбора датасета нами был созданы две идентичные мобильные установки -- фотоаппараты с закрепленными на них цветовыми мишенями, показанные на рисунке \ref{fig:mobile}.
}
{
We created two identical handheld setups to collect the dataset in natural (uncontrolled) conditions.
Cameras with color targets mounted on them are shown in Fig.~\ref{fig:mobile}.
}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\linewidth]{images/mobile_setup.jpg}
    % \center{{\bf Figure 4.}Two mobile installations for collecting data in uncontrolled conditions.}
    \caption{Two handheld setups for collecting data in uncontrolled conditions.}
    
    \label{fig:mobile}
\end{figure}

\ruengtext{
Одним из ключевых факторов при формировании датасета является консистентность между освещенностью цветовой мишени и наблюдаемой сценой: важно, чтобы один и тот же источник (или пара источников) освещали как всю сцену, так и цветовую мишень, иначе полученная оценка будет нерелевантна большей части сцены.
Такие ситуации могут возникать, когда локальное освещение около фотографа не совпадает с освещением снимаемой сцены (примеры представлены на рисунках 5а-в).
}
{
One of the key factors in the dataset collection is the consistency between the illumination of the color target and the observed scene.
The same source (or a pair of sources) must illuminate both the entire scene and the color target.
Otherwise, the source color estimation will be irrelevant to the most pixels of the scene.
Such situations occur when the local illumination near the photographer does not match the illumination of the scene being shot 
(examples are shown in Fig.~\ref{fig:examples}a-c).
}

\begin{figure}[h]
\center
\begin{minipage}[h]{0.23\linewidth}
\center{\includegraphics[width=1\linewidth]{images/IMG_8162.JPG} \\ (a)}
\end{minipage}
\begin{minipage}[h]{0.23\linewidth}
\center{\includegraphics[width=1\linewidth]{images/IMG_8586.JPG} \\ (b)}
\end{minipage}
\begin{minipage}[h]{0.23\linewidth}
\center{\includegraphics[width=1\linewidth]{images/IMG_8674.JPG} \\ (c)}
\end{minipage}
\begin{minipage}[h]{0.23\linewidth}
\center{\includegraphics[width=1\linewidth]{images/IMG_8496.JPG} \\ (d)}
\end{minipage}

% \center{ {\bf Figure 5.}
\caption{
Examples of photographs that should be excluded from the dataset: 
a) the color target is illuminated by a lantern, the color of which is different from the lighting of the building;
b) the lighting of the cube's borders is the result of multiple reflections in a room with almost white walls;
c) the color target is illuminated by sources that have almost no effect on the lighting of the observed scene;
d) the majority of the color target pixels are clipped white due to overexposure.
\label{fig:examples}
}
\end{figure}

\ruengtext{
Другим немаловажным фактором является наличие бликов на цветовой мишени. 
Для тех изображений, где для тёмно-серых граней наблюдается зашкаливание значений в каком-то из каналов, невозможно извлечь корректную оценку освещения (пример на рисунке 5г). 
Для того, чтобы избегать возникновения таких изображений, следует либо использовать ручные настройки, либо в настройках камеры указать затемнение относительно автоматической оценки экспозиции. 
В нашем случае обычно хватает затемнения на одну ступень.%ограничивать максимально допустимую чувствительность. 
Отдельно стоит подчеркнуть важность правильного фотографирования сцен с двумя источниками освещения.
Крайне желательно, особенно если площади изображения сцены, освещенной разными источниками освещения, сопоставимы, расположить цветовую мишень так, чтобы цвета разных её граней заметно отличались.
Используя такую разметку, возможно оценить нормаль к плоскости в пространстве цветов, задаваемой цветами левой и правой граней, контролируя тем самым оценку сразу двух значимых источников освещения. 
}{
Another important factor is the presence of glare on the color target. 
For those images where for dark gray faces of the color target there are clipped values in one of the channels,
it is impossible to extract a correct illumination estimation (an example is presented in Fig.~5d). 
To avoid such images, one should consider either manual camera settings or specifying relative exposure compensation to camera automatic estimation. 
In our case, dimming by one step is usually enough. 
Separately, we should note the importance of correct photography of scenes with two light sources. 
It is highly recommended, especially if the image areas of the scene illuminated by different light sources are comparable, place the color target so that the colors of its different faces noticeably differ. In this case, it is possible to estimate the plane in the color space containing the colors of the left and right sides, thereby the evaluation of two significant light sources is controlled at once.
}

% :(


\ruengtext{
Наконец, как было сказано ранее, целесообразно выполнять дополнительную семантическую разметку содержимого сцены на изображениях. 
В настоящий момент предлагается следующая иерархия признаков:
\begin{enumerate}
    \item Время дня (день/ночь/неизвестно)
    \item Место (улица/помещение)
    \item Наличие источника в кадре (солнце/небо/лампы/фонари)
    \item Наличие объектов, которые можно идентифицировать (лица/номера ТС и др.)
    \item Наличие в сцене объектов известной окраски
    \item Наличие теней (есть/нет)
    \item Богатство сцены (богатая/бедная/непонятно)
    \item Основное освещение (солнце/небо/лампа/фонарь/непонятно)
\end{enumerate}
}
{
As shown, additional semantic markup of the scene content is valiable. So we propose the following feature hierarchy:
\begin{enumerate}
    \item Time of day (day/night/unknown)
    \item Location (indoor/outdoor)
    \item The presence of light source in the frame (sun/sky/lamps/street lights)
    \item The presence of objects that can be identified (human faces/license plates, etc.)
    \item The presence of objects of known color in the scene
    \item The presence of shadows (yes/no)
    \item The richness of the scene (rich/poor/unclear) 
    \item Main lighting (sun/sky/lamp/lantern/unclear)
\end{enumerate}
}

\ruengtext{
Список является не завершенным, однако представляется, что с его помощью возможно профилировать различные алгоритмы оценки освещения, выявляя трудные сценарии. 
}{
The hierarchy is incomplete, but currently, it can profile various illumination estimation algorithms and identify challenging scenarios.
}


==> chapters/color_targets.tex <==
\section{Color targets}

\ruengtext{
Большинство современных и признанных датасетов используют плоские цветовые мишени разных производителей, к таким датасетам относятся: NUS \cite{cheng2014illuminant}, REC \cite{hemrit2018rehabilitating}, INTEL-TUT \cite{aytekin2019tut}, INTEL-TAU \cite{laakom2019tau}, MLS \cite{sma}. 
}{
Most modern and well-known datasets use flat color targets of different manufacturers, such datasets include: NUS \cite{cheng2014illuminant}, REC \cite{hemrit2018rehabilitating}, INTEL-TUT \cite{aytekin2019tut}, INTEL-TAU \cite{laakom2019tau}, MLS \cite{sma}.
}

\ruengtext{
Как было сказано выше, с помощью плоской цветовой мишени невозможно корректно оценить освещения в случае наличия двух значимых источников освещения сцены (заметим, что речь идет не только о фотографиях, сделанных ясным днем, но и о множестве изображений с различными источниками искусственного освещения, как на улице, так и в помещении). 
С другой стороны, преимуществом цветовых мишеней является то, что они пригодны не только для оценки точности определения освещения, но и для оценки качества решения в задачах цветовой коррекции и перехода в пространство стандартного наблюдателя XYZ. 
Нельзя также не отметить, что именно плоские цветовые мишени обычно изготавливаются по самым высоким стандартам точности.
}
{
As mentioned above, it is impossible to correctly estimate light source using a flat color target if two significant sources of illumination are present in the scene (note: this applies not only to photographs taken on a clear day but also to a multitude of images with various artificial light sources taken in the night street as well as indoors). 
On the other hand, the advantage of color targets is that they are suitable not only for the evaluation of illumination estimation accuracy, but also for the quality evaluation of problem solution of color correction, and for a transition to the XYZ color space. 
It should also be noted that specifically flat color targets are usually manufactured with the highest standards of precision.
}

\ruengtext{
Среди объемных цветовых мишеней, которые использовались для формирования датасетов, можно перечислить всего две: серый шар (как в датасете GrayBall \cite{ciurea2003large}) и SpyderCube (CubePlus \cite{banic2017unsupervised}). Можно также представить использование нескольких плоских цветовых мишеней для этой цели, так некоторые плоские цветовые мишени изготавливаются для компактности в складывающемся виде. 
Однако подобные публичные датасеты на данный момент авторам не известны. 
}
{
Among three-dimensional color targets that were used in datasets, only two can be listed: a gray ball (as in the GrayBall \cite{ciurea2003large} dataset) and SpyderCube (CubePlus \cite{banic2017unsupervised}).
It is quite possible to use several flat color targets or flat color targets, which are made foldable for compactness, to reach 3D quality.
However, such public datasets are currently unknown to the authors.
}

\ruengtext{
Вообще говоря, серый шар представляется более удачной, чем SpyderCube, цветовой мишенью, поскольку позволяет выполнять более полную оценку освещения. 
Во-первых анализируя гистограмму цветов пикселей изображения серого шара возможно непосредственно оценить число источников (ранг освещения), если их не больше трех.
Конкретнее, если ненулевые значения на гистограмме укладываются на одну прямую, то у сцены один источник, если на плоскость -- два, если достаточно полно заполнена вся гистограмма -- три. 
Во-вторых, помимо анализа гистограммы, можно анализировать тени на данном шаре, что позволяет увеличить максимальный ранг освещения, который можно оценить \cite{bouganis2004multiple}.
}
{
Generally, a gray ball seems to be a better color target than SpyderCube, since it allows a more detailed illumination estimation. 
First, by analyzing the histogram of the pixels' colors in the image of a gray ball, it is possible to estimate the number of sources (illumination rank) directly, if there are no more than three of them. 
Specifically, if non-zero values on the histogram fit into one straight line, then the scene has one source, if it fits on the plane -- two, if the entire histogram is densely filled -- then there are three sources. 
Secondly, in addition to the histogram analysis, the shadows on this ball can be considered, which allows increasing the maximum illumination rank, which can be estimated \cite{bouganis2004multiple}.
}

\ruengtext{
Несмотря на вышесказанное, в сложившейся ситуации выбирать серый шар в качестве цветовой мишени -- не лучшее решение.
Во-первых, потому, что существующий датасет уже достаточно сильно устарел (он был собран в 2003 году), во-вторых, на рынке не представлены цветовые мишени со стабильными цветовыми характеристиками в виде серого шара.
}
{
Despite the above, choosing a gray ball as a color target currently is not the best solution. The existing dataset collected in 2003 is already outdated, and color targets in the form of a gray ball with stable color characteristics are not available on the market.
}

%\afterpage{
\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\textwidth]{images/SpyderCube_GeneralView.jpg}
    % \center{{\bf Figure 3.} SpyderCube color target by DataColor\footnotemark.}
    \caption{SpyderCube color target by DataColor\protect\footnotemark.}
    \label{fig:spydercube}
\end{figure}
% \todo{не забыть пофиксить проблему с footnote}

\footnotetext{Image from \href{https://www.displaydaily.com/index.php?option=com_content&view=article&id=50684:cinematography-hdr-and-waveform-monitors}{displaydaily.com}}

\ruengtext{
В том числе поэтому для создания наиболее репрезентативного и самого большого среди существующих датасетов целесообразно использовать SpyderCube фирмы DataColor (рисунок \ref{fig:spydercube}), поскольку для него уже собрано около 2000 изображений, а также поскольку с его помощью можно определить плоскость на цветовой гистограмме, содержащей цвета источников.
В добавок к этому использование SpyderCube позволяет работать с различными уровнями яркости: для лучшей оценки в темноте есть белые области на гранях, для ярких сцен -- серые. 
Есть также имитация абсолютно черного тела (отверстие в основании), по которому можно оценить уровень черного и, наконец, зеркальный шарик сверху в сжатом виде содержит информацию о мире, расположенном над сценой, в том числе о других источниках освещения. 
}
{
Hence, it is advisable to use Datacolor's SpyderCube (Fig.~\ref{fig:spydercube}) to create the most representative and largest dataset among existing ones  -- about 2000 images have already been collected with it, and this target makes it possible to determine the plane on the color histogram that contains the sources' colors. 
Besides, SpyderCube can be used in a wide range of exposures: % dynamic range, exposure latitude?
there are white areas on the edges for dark scenes estimation, 
and gray areas for bright scenes. 
It also contains an imitation of a completely black body (a hole in the base), that can be used to estimate the camera's black level. 
Finally, the mirror ball at the top contains information about the world above the scene in a compressed form, including information about other light sources.
}


==> chapters/conclusion.tex <==
\section{Conclusion}

In this article, we discuss the main pros and cons of the largest datasets available for the light source estimation problem. We present a brief analysis of three-dimensional color targets and highlight some of the technical and scientific details that we discovered when collecting our new dataset. We provide typical examples of images with the incorrectly illuminated color target and, finally, suggest relevant image categorization.

The collected dataset will be used in the upcoming 2-nd Illumination Estimation Challenge (IEC 2020) starting 1-st July 2020 and organized by the Institute for Information Transmission Problems (IITP RAS) in cooperation with University of Zagreb, see \url{http://chromaticity.iitp.ru}.

We are pleased to invite all interested teams to participate in the competition.

% \ruengtext{
% В работе проведен анализ различных цветовых мишеней, а также освещены некоторые технические и научные тонкости, существенные при формировании датасета для оценки освещения сцены. 
% }{
% In this work, we discussed the pros and cons of the existing datasets for collor we presented various color targets analysis, that highlighted some technical and scientific details, which are significant in the process of collecting datasets for light source estimation.  and the features we desire for our new dataset.
% }

% % \ruengtext{
% % С точки зрения представленного анализа, а также опыта формирования собственного датасета, обсуждены достоинства и недостатки существующих датасетов.
% % }{


% % % From the presented analysis and experience collecting our own dataset, we have discussed the advantages and disadvantages of existing datasets. 
% % }

% \ruengtext{
% Собираемый датасет будет использован в предстоящем международном соревновании по цветовой константности, который будет проводиться Институтом Проблем Передачи Информации (ИППИ РАН) летом 2020 года.
% Авторы будут рады видеть в составе участников всех желающих.
% }
% {
% The collected dataset will be used in the upcoming 2-nd Illumination Estimation Challenge (IEC 2020) starting 1-st July 2020 organized by the Institute for Information Transmission Problems (IITP RAS), see \url{http://chromaticity.iitp.ru}.
% }

% \ruengtext{}{
% We are pleased to invite all interested teams to participate in the competition.
% }

%Помимо вышеперечисленного данная работа также преследует рекламную цель, а именно -- анонс предстоящего международного соревнования по цветовой константности, организуемого Институтом Проблем Передачи Информации (ИППИ РАН), который будет проводиться летом 2020 года. 



==> chapters/intro.tex <==
\section{Introduction}

\ruengtext{
Оценка освещения -- это неотъемлемый этап цветового конвейера формирования изображений в современных мобильных устройствах. 
В настоящее время классический и устоявшихся подход к визуализации изображений, снятых цифровой камерой, подразумевает обязательное наличие в нём трех этапов \cite{brown2016pipeline}: оценка освещения, коррекция освещения и переход в цветовое пространство CIE XYZ \cite{nikol}.
Считается, что, оперируя цветами в CIE XYZ (цветовое пространство стандартного наблюдателя), возможно достичь лучшего качества цветовоспроизведения, так называемой фотореалистичности. 
Следует отметить, что при съемках изображений современными мобильными камерами фотореалистичность как цель зачастую уступает место эстетичности, однако обычно это достигается без исключения вышеупомянутых трех этапов.
}
{
Light source estimation is an essential part of the color image formation pipeline in modern mobile devices. 
Currently, the classic and well-established approach to digital camera images visualization includes three necessary stages \cite{brown2016pipeline}: illumination estimation, illumination correction, and conversion to the CIE XYZ color space (CIE standard observer color space) \cite{nikol}. 
The usual assumption is that  CIE XYZ color space leads to a better quality of color reproduction or ``photorealism''. 
However, photorealism as a goal is often abandoned for aesthetics while taking pictures with modern mobile cameras, but the above three stages usually are preserved.
}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\linewidth]{images/frequency_all_2.png}
    % \center{{\bf Figure 1.} The annual number of open dataset publications on the topic of color constancy.}
    \caption{The annual number of open dataset publications on the topic of color constancy.}
    \label{fig:frequency}
\end{figure}
%\FloatBarrier

\ruengtext{
Другим свидетельством актуальности задачи оценки освещения сцены является частота публикации открытых датасетов (наборов данных) по этой тематике: начиная с 2002 года в среднем каждый год публикуется не менее одного нового датасета (рисунок \ref{fig:frequency})\footnote{Эта статистика получена преимущественно на основе сведений сетевого ресурса \href{https://colorconstancy.com}{colorconstancy.com}}. 
С другой стороны такая активность свидетельствует и о том, что в мировом научном сообществе стандарт оценки качества этой задачи ещё не сформирован (как это произошло, например, в задаче стереосопоставления \cite{szeliski2002taxonomy}).
}{
Continued publication of open datasets on this topic is further evidence of the importance of this task. 
Since 2002, on average, there is at least one new dataset every year 
(Fig.~\ref{fig:frequency})\footnote{These statistics were obtained mainly via the network resource \href{https://colorconstancy.com}{colorconstancy.com}}. 
Such activity also indicates that standard methods for assessing the quality of this particular problem solution have not yet been formed in the world scientific community (as happened, for example, in the task of stereo correspondence algorithms evaluation \cite{szeliski2002taxonomy}).
}

% On the other hand, such activity also indicates that a standard for assessing the quality of this particular problem solution has not yet been formed in the world scientific community (as happened, for example, in the task of stereo correspondence algorithms evaluation \cite{szeliski2002taxonomy}).


\ruengtext{
В прошлом году был опубликован большой датасет IntelTAU \cite{laakom2019tau}. 
Он решает несколько проблем представленных ранее датасетов, однако у него есть свои недостатки, не позволяющие ему занять нишу <<стандартного>>, которые обсуждаются ниже. 
Другой достаточно большой и разнообразный датасет, также представленный в прошлом году, -- это CubePlus \cite{banic2017unsupervised}.
Данный датасет использовался для проведения международного соревнования по оценке освещения в 2019 году. 
Но, как показал опыт, и он имеет свои недостатки.
}{
A large IntelTAU dataset was published last year \cite{laakom2019tau}. 
It solves several problems with previously presented datasets. However, it has drawbacks (discussed below) that prevent it from occupying the “standard” niche. Another quite large and diverse dataset, also introduced last year, is CubePlus \cite{banic2017unsupervised}. 
This dataset was used for the first international illumination estimation challenge in 2019. 
Nevertheless, as we will see, it is also not perfect.
}

\ruengtext{
В данной работе предлагается некоторый содержательный анализ проблем существующих цветовых мишеней, а также перечисляются технические и научные трудности с которыми приходится сталкиваться в процессе подготовки нового датасета. 
}
{
This paper proposes some meaningful analysis of the existing color targets problems. It lists the technical and scientific difficulties encountered in preparing a new dataset for the 2-nd Illumination Estimation Challenge starting 1-st July 2020, which is organized by the Institute for Information Transmission Problems (IITP RAS) in cooperation with University of Zagreb, Croatia.
}

\ruengtext{
Стоит отметить, что эта статья в том числе является приглашением к участию в новом соревновании по оценке освещенности сцены, организуемом Институтом Проблем Передачи Информации (ИППИ РАН), которое будет проходить этим летом. 
}
{
We also invite anyone to participate in this competition for scene illumination estimation, see \url{http://chromaticity.iitp.ru}.
}

\section{Disadvantages of the modern datasets}

\ruengtext{
Рассмотрим один из последних датасетов -- IntelTAU \cite{laakom2019tau}. 
Авторы данного датасета отмечают его преимущества по сравнению с предшественниками.
}{
Let us consider one of the latest datasets -- IntelTAU \cite{laakom2019tau}.
The authors of this dataset point out its advantages compared to the predecessors.
}

% \todo 6 тысяч изображений!
% В качестве подтверждения последнего утверждения рассмотрим последний из опубликованных наборов данных INTEL-TAU \cite{laakom2019tau}. 
\ruengtext{
    \begin{itemize}
        \item \textbf{Большое количество изображений}. IntelTAU считается самым большим, в нём чуть более семи тысяч изображений: три тысячи с одной из камер и по две с двух других. Однако многие изображения содержат сильно пересекающиеся сцены.
        \item \textbf{GDPR-совместимость}. Данный датасет удовлетворяет требованиям европейских норм по защите персональных данных. Изображения не содержат приватной информации, такой как лица и номера автомобилей 
        \item \textbf{Разнообразие камер}. Изображения получены с трёх камер, что позволяет тестировать устойчивость алгоритма к смене сенсора. 
        \item Авторы подчеркивают \textbf{отсутствие калибровочных объектов в кадре}. Изображения с цветовой  мишенью были получены отдельно и в датасете почти не представлены.
    \end{itemize}
}{
    \begin{itemize}
        \item \textbf{A large number of images.} IntelTAU is considered to be the largest dataset, with just over seven thousand images: three thousand from one of the cameras and two thousand from each of two other cameras.
        \item \textbf{GDPR compatibility.} This dataset meets the requirements of European standards for personal data protection. Images do not contain private information, such as faces and license plates.
        \item \textbf{A variety of cameras.} Images were obtained from three cameras with different sensors, which allows testing the stability of the algorithm to sensor changes.
        \item The authors highlight \textbf{the absence of calibration objects in the frame}. Images with a color target were obtained separately and are almost not represented in the dataset.
    \end{itemize}
}

\ruengtext{
С последним пунктом, однако, трудно согласиться, поскольку авторы предоставляют свои оценки освещения для изображений без цветовых мишеней.
Получается, что нельзя проверить качество аннотации, а опыт показывает, как это важно: в одном из самых популярных датасетов продолжают находить и исправлять ошибки разметки \cite{hemrit2018rehabilitating} -- наличие цветовой мишени в кадре позволяет уменьшить влияние человеческого фактора.
}{
However, it is difficult to agree with the last point, since the authors provide their own light source estimations for images without color targets. It turns out it is impossible to evaluate the quality of the annotation, and experience shows just how important this verification is: in one of the most popular datasets, markup errors are  found continuously and corrected \cite{hemrit2018rehabilitating} -- the presence of a color target in the frame allows for the human factor influence reduce.
}

\ruengtext{
Также с целью удовлетворить условиям GDPR в данном датасете лица были размыты.
Из-за этого многие изображения являются несколько искусственными, что может повлиять на применение методов, основанных на машинном обучении.
Есть и другие недостатки, в том числе свойственные многим другим датасетам.
}{
Also, in order to meet the GDPR conditions, the faces were blurred in this dataset. Thus, many images are somewhat artificial, which may affect the use of methods based on machine learning. There are other disadvantages, including those common among many other datasets.
}

%Следующее обстоятельство, на которое следует обратить внимание, -- это формат предоставляемой разметки.

\ruengtext{
Многие датасеты, в том числе IntelTAU, измеряют освещенность с использованием плоской цветовой мишени (рисунок \ref{fig:colorchecker}). 
Используя плоскую цветовую мишень возможно выполнить только оценку освещения одним источником, но что это будет за оценка, скажем, в ясный солнечный день? 
В случае, если цветовая мишень находится в тени (не освещена солнцем), то единственным источником освещения будет небо, которое является существенно менее ярким источником освещения сцены, нежели солнце. 
В случае же, если цветовая мишень не в тени, то на неё падает одновременно освещение от солнца и неба, то есть измерена некоторая смесь двух источников. 
В результате получается, что алгоритмы и модели, обученные на таких датасетах решают достаточно непонятную задачу для изображений, сделанных солнечным днем: предсказать некоторую линейную комбинацию цветов двух источников освещения, веса которых взяты в неизвестной пропорции.
Устранить этот недостаток можно только с помощью объёмных цветовых мишеней, как, сделано, например, в датасете \cite{ciurea2003large}. 
Хорошим современным примером подобного датасета является CubePlus \cite{banic2017unsupervised}).
}{
Many datasets, including IntelTAU, estimate illumination using a flat color target (Fig.~\ref{fig:colorchecker}).
With a flat color target, it is possible to perform only a single light source estimation, but what kind of estimation will it be, say, on a clear sunny day? 
If the color target is in the shadow (not illuminated by the sun), the only light source will be the sky,
which is usually a significantly less bright light source than the sun. 
If the color target is not in the shadow, then the sun and sky are light sources acting simultaneously.
Hence, the mixture of two sources is estimated. 
As a result, the algorithms and models trained on such datasets solve quite an incorrect problem
for images taken on a sunny day: to predict a precise linear mixture of colors of two light sources with unknown proportions.
This drawback can only be eliminated with the help of the three-dimensional color targets,
as was done, for example, in the \cite{ciurea2003large} dataset.
One good modern example of such a dataset is CubePlus \cite{banic2017unsupervised}).
}

\ruengtext{
Помимо вышеперечисленных проблем стоит выделить ещё три недостатка, характерные для всех существующих датасетов.
}{
In addition to the above problems, there are three more drawbacks that are characteristic of all existing datasets.
}

\ruengtext{
\begin{enumerate}
    \item \textbf{Отсутствие дополнительной аннотации}. Сопутствующая информация по типу сцены, времени дня, наличию объектов известной окраски и другим семантическим признакам важна для алгоритмов цветовой константности.
    Она бы позволила не только определять одно число -- качество решения для всех изображений, но и анализировать профиль ошибки по различным категориям.
    Например, оценка освещения хорошо выполняется для фотографий естественного дневного освещения, а для искусственного -- нет.
    \item \textbf{Недостаточное количество изображений}. Даже в рекордном для данной задачи датасете IntelTAU содержится не более трёх тысяч фотографий на один сенсор, зачастую по нескольку изображений одной и той же сцены. 
    Тем более это относится к не столь новым датасетам. 
    Например, в классическом датасете для оценки освещения ColorChecker \cite{hemrit2018rehabilitating} меньше тысячи изображений. 
    Такое количество может быть не достаточно для разработки алгоритмов цветовой константности, рассчитанных на разнообразные типы сцен.
    % Следовательно некоторые содержательные и удачные улучшения следующей версии разрабатываемого алгоритма можно просто не заметить, поскольку датасет содержит небольшое количество соответствующих решаемой проблеме примеров. 
    \item \textbf{Несовместимость датасетов}. 
    Зачастую каждый следующий датасет собирается с помощью камеры, отличной от предыдущих, а цветовые мишени тоже разнятся.
    В связи с этим проблемно объединять накопленные датасеты в один большой. 
    В этой ситуации затруднительно установить причину ошибки алгоритма -- была ли это действительно сложная сцена или же причина в том, что характеристики чувствительности данной камеры отличались от тех, что использовались на стадии разработки алгоритма. Редкими примерами согласованного дополнения датасета являются CubePlus, продолжающий датасет Cube, и IntelTAU, продолжающий IntelTUT 
\end{enumerate}
}
{
\begin{enumerate}
    \item \textit{No additional annotation.}
    Related information on the type of scene, time of day, the presence of objects of known color, and other semantic features are valuable for color constancy algorithms. Such information could allow not only to calculate the aggregated value -- the quality of the solution for all images but also to analyze the error clusters. For example, a specific light source estimation algorithm can work well for images shot in natural daylight conditions but not in artificial lighting.
    \item \textit{Insufficient number of images.} 
    Even a record-setting IntelTAU dataset contains no more than three thousand photos per sensor, which often contains repeated images of the same scene; moreover, this applies to older datasets as well. 
    For example, a classic dataset for light source estimation, ColorChecker \cite{hemrit2018rehabilitating}, has less than a thousand images. 
    Such a limited quantity may not be enough to develop color constancy algorithms designed for various types of scenes. 
    \item \textit{Incompatibility of datasets.} 
    Each subsequent dataset is often collected using a camera different from the ones used to collect previous datasets, and color targets may also differ.  
    Thus, it is problematic to combine the accumulated datasets into one. 
    In this situation, it is difficult to analyze the source of the algorithm error -- 
    was it a complexity of the scene, or was it because the camera's sensitivity characteristics were different from those used at the algorithm development stage?
    Rare examples of consistent dataset additions are CubePlus, which expands the Cube dataset, and IntelTAU, which expands IntelTUT.
\end{enumerate}
}

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{images/colorchecker_intel_tau.jpg}
    \caption{ Example of a flat color target. The image was taken from the IntelTAU dataset.}
    \label{fig:colorchecker}
\end{figure}
%\FloatBarrier

\ruengtext{
Одним из возможных вариантов решения вышеперечисленных проблем является существенное пополнение и аннотация одного из современных больших и содержащих объемную цветовую мишень датасетов.
Именно этого подхода придерживаются авторы, взяв за основу датасет CubePlus.
}{
A possible solution to the above problems is to substantially expand and annotate one of the large modern datasets containing a three-dimensional color target.
The authors adhere to this approach using the CubePlus dataset as a basis.
}
